Approximation Algorithms for Coordinating Ad Campaigns on Social Networks

We study a natural model of coordinated social ad campaigns over a social network, based on models of Datta et al. and Aslay et al. Multiple advertisers are willing to pay the host - up to a known budget - per user exposure, whether the exposure is sponsored or orgain (i.e. shared by a friend). Campaigns are seeded with sponsored ads to some users, but no user must be exposed to too many sponsored ads. Thus, while ad campaigns proceed independently over the network, they need to be carefully coordinated with respect to their seed sets. We study the objective of maximizing host's total ad revenue. Our main result is to show that under a broad class of influence models, the problem can be reduced to maximizing a submodular function subject to two matroid constraints; it can therefore be approximated within a factor essentially 1/2 in polynomial time. When there is no bound on the individual seed set sizes of advertisers, the constraints correspond only to a single matroid, and the guarantee can be improved to 1-1/e; in that case, a factor 1/2 is achieved by a practical greedy algorithm. The 1-1/e approximation algorithm for matroid-constrained problem is far from practical; however, we show that specifically under the Independent Cascade model, LP rounding and Reverse Reachability techniques can be combined to obtain a 1-1/e approximation algorithm. Our theoretical results are complemented by experiments evaluating the extent to which the coordination of multiple ad campaigns inhibits the revenue obtained from each individual campaign, as a function of the similarity of the influence networks and strength of ties in the networks. Our experiments suggest that as networks for different advertisers become less similar, the harmful effect of competition decreases. With respect to tie strengths, we show that the most harm is done in an intermediate range.

==> app-lp-rounding.tex <==
In this section, we provide additional details on the dependent
LP-rounding algorithm of
Gandhi et al.~\cite{gandhi:khuller:parthasarathy:srinivasan:dependent},
and a way to simplify and speed up the algorithm when there are no
constraints on the seed set sizes of individual advertisers.

The algorithm of Gandhi et al.~can be applied to round fractional
solutions whenever the variables to be rounded (here: the
\Select[j]{v}) can be considered as edges in a bipartite graph,
and constraints correspond to bounds on the (fractional) degrees of the
nodes of the bipartite graph.\footnote{%
The fifth constraint of our LP (overall budget) does not fit in
this framework, since it is a constraint on all variables.
We extend the rounding algorithm of Gandhi et al.~by one more final
loop (see below) which repeatedly picks any two fractional variables
and randomly rounds them using the same approach as the rest of the algorithm, 
until only one fractional variable remains.
This last variable can then be rounded randomly by itself.}
It repeatedly rounds the fractional values associated with a subset of
edges forming a maximal path or a cycle,
until all variables are integral;
let \ISelect[j]{v} denote the rounded (integral) values corresponding
to \Select[j]{v}.
The algorithm of \cite{gandhi:khuller:parthasarathy:srinivasan:dependent}
provides the following guarantees:
\begin{itemize}
\item The probability that the variable \Select[j]{v} is rounded to
  $\ISelect[j]{v} = 1$
  is exactly \Select[j]{v}, for all $j$ and $v$.
\item In the bipartite graph, each node's degree is rounded up or down
to an adjacent integer.
In the context of our LP~\eqref{eqn:ILP},
this means that the number of seed nodes for each advertiser is either
rounded up or down to the nearest integer,
as is the number of exposures to sponsored ads for each node.
In particular, the third and fourth constraints are satisfied with
probability 1.
\item For any node of the bipartite graph and any subset of incident
edges, the rounded values are negatively correlated.
In the context of our LP~\eqref{eqn:ILP},
for any advertiser $j = j(i)$ and reverse reachable set $R_i$, 
the algorithm guarantees that
$\Prob{\ISelect[j]{v} = 0 \text{ for all } v \in R_i}
\leq \prod_{v \in R_i} \Prob{\ISelect[j]{v} = 0}
= \prod_{v \in R_i} (1-\Select[j]{v})$.
\end{itemize}

After rounding all the \Select[j]{v} to \ISelect[j]{v},
for each $i$, we set
$\ISSel{i} = 1$ if at least one $v \in R_i$ has $\ISelect[j(i)]{v} = 1$,
and for each $j$, we set
$\IRev[j] = \sum_{i \in \RRP[j]} \PER[j] \cdot \ISSel{i}$.
Together with the guarantees of Gandhi et al., this ensures that 
all ILP constraints except possibly the seventh (budget) constraint
are satisfied; the budget constraint is discussed more in
Section~\ref{sec:budget-constraints}.

We now derive the approximation guarantee.
Consider any set $R_i \in \RRP[j]$.
With explanations of some steps given below,
the probability that $\ISSel{i} = 1$ is
\begin{align*}
\Prob{\ISSel{i} = 1}
    & = 1 - \Prob{\ISelect[j(i)]{v} = 0 \text{ for all } v \in R_i}
\\  & \stackrel{(1)}{\geq} 1 - \prod_{v \in R_i} \Prob{\ISelect[j(i)]{v} = 0}
\\  & = 1 - \prod_{v \in R_i} (1-\Select[j(i)]{v})
\\  & \stackrel{(2)}{\geq} 1 - \e^{-\sum_{v \in R_i} \Select[j(i)]{v}}
\\  & \geq 1 - \e^{-\min(1, \sum_{v \in R_i} \Select[j(i)]{v})}
\\  & \stackrel{(3)}{\geq} (1-1/\e) \cdot \min(1, \sum_{v \in R_i} \Select[j(i)]{v})
\\  & \stackrel{(4)}{\geq} (1-1/\e) \cdot \SSel{i}.
\end{align*}

The inequality labeled (1) used the negative dependence discussed above.
The inequality labeled (2) used the standard bound that $1-x \leq
\e^{-x}$ for all $x \geq 0$.
The inequality labeled (3) uses that the function
$x \mapsto 1-\e^{-x}$ is concave,
and hence on the interval $[0,1]$ is lower-bounded by the straight
line which agrees with it at the endpoints $x=0$ and $x=1$,
which is the function $x \mapsto (1-1/\e) \cdot x$.
Finally, the inequality labeled (4) uses that
$\SSel{i} \leq \min(1, \sum_{v \in R_i} \Select[j(i)]{v})$
by the first and second LP constraints.
Using the definition of \IRev[j], we now get that

\begin{align*}
\Expect{\IRev[j]}
& = \Expect{\sum_{i \in \RRP[j]} \PER[j] \cdot \ISSel{i}}
\; = \; \sum_{i \in \RRP[j]} \PER[j] \cdot \Prob{\ISSel{i} = 1}
\\ & \geq \sum_{i \in \RRP[j]} \PER[j] \cdot (1-1/\e) \cdot \SSel{i}
\; \geq \; (1-1/\e) \cdot \Rev[j].       
\end{align*}

% \subsection{No Seed Set Size Restrictions}
% \label{sec:unrestricted-seed-sets}
% In the model of Aslay et al.,
% and in our experiments in Section~\ref{sec:experiments}, 
% there are no restrictions placed on the seed set sizes of individual
% advertisers;
% that is, the fourth set of constraints in the LP~\eqref{eqn:ILP}
% is missing.
% Then, except for the fifth (sum of seed set sizes) constraint,
% the \Select[j]{v} constraints are a collection of disjoint stars.
% As a result, the general correlated rounding algorithm of Gandhi et
% al.~can be replaced with their algorithm for stars.
% The resulting algorithm runs in linear time and is very simple to implement.
% It first uses the correlated rounding on pairs of variables
% \Select[j]{v}, \Select[j']{v} corresponding to the same 
% node (and different advertisers) until no such pairs remain;
% subsequently, as for the general algorithm,
% we add one more \textbf{while} loop to round pairs of the remaining
% \Select[j]{v} (which now necessarily correspond to distinct nodes $v,v'$).

% Because there is at most one fractional variable remaining incident on
% any node $j$ or $v$, the second property of the Gandhi et al.~rounding
% algorithm is preserved.
% The negative correlation property holds inductively,
% because at most two values are rounded in each step.

% \begin{algorithm}
% \caption{The dependent LP rounding algorithm.\label{algo:rounding}}
% \begin{algorithmic}[h]
% \WHILE{there are $v, j, j'$
%   with $j \neq j'$ and $\Select[j]{v}, \Select[j']{v} \in (0,1)$}
% \STATE Let $\delta = \min(\Select[j]{v}, 1-\Select[j']{v})$
%        and $\delta' = \min(\Select[j']{v}, 1-\Select[j]{v})$.
% \STATE Flip a coin with bias $\frac{\delta}{\delta+\delta'}$.
% \IF{it comes up heads}
% \STATE Round $\Select[j]{v} := \Select[j]{v} + \delta'$
%   and $\Select[j']{v} := \Select[j']{v} - \delta'$.
% \ELSE
% \STATE Round $\Select[j]{v} := \Select[j]{v} - \delta$
%   and $\Select[j']{v} := \Select[j']{v} + \delta$.
% \ENDIF
% \ENDWHILE
% \WHILE{there are $v, v' j, j'$
%   with $v \neq v'$ and $\Select[j]{v}, \Select[j']{v'} \in (0,1)$}
% \STATE Let $\delta = \min(\Select[j]{v}, 1-\Select[j']{v'})$
%        and $\delta' = \min(\Select[j']{v'}, 1-\Select[j]{v})$.
% \STATE Flip a coin with bias $\frac{\delta}{\delta+\delta'}$.
% \IF{it comes up heads}
% \STATE Round $\Select[j]{v} := \Select[j]{v} + \delta'$
%   and $\Select[j']{v'} := \Select[j']{v'} - \delta'$.
% \ELSE
% \STATE Round $\Select[j]{v} := \Select[j]{v} - \delta$
%   and $\Select[j']{v'} := \Select[j']{v'} + \delta$.
% \ENDIF
% \ENDWHILE
% \FOR{all $j,v$}
% \STATE Let $\ISelect[j]{v} = 1$ with probability \Select[j]{v},
% and $\ISelect[j]{v} = 0$ otherwise.
% \ENDFOR
% \FOR{all $i$}
% \STATE Let $\ISSel{i} = 1$ if at least one $v \in R_i$ has
% $\ISelect[j(i)]{v} = 1$.
% \ENDFOR
% \FOR{all $j$}
% \STATE Let $\IRev[j] = \sum_{i \in \RRP[j]} \PER[j] \cdot \ISSel{i}$.
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}

% To prove the feasibility of the output $(\ISSelV, \IRevV, \ISelectV)$
% of Algorithm~\ref{algo:rounding} --- except for the budget
% constraints, which are discussed in more depth in
% Section~\ref{sec:budget-constraints} --- 
% we observe the following properties:
% \begin{enumerate}
% \item Throughout the first \textbf{while} loop, the sum
%   $\sum_j \Select[j]{v}$ stays constant for each $v$.
%   This is because when some amount is added to one variable, the same
%   amount is subtracted from another.
%   As a consequence, the sum of \emph{all} \Select[j]{v} also stays
%   constant.
  
%   Similarly, throughout the second \textbf{while} loop, the sum of
%   all \Select[j]{v} stays constant.
% \item The definition of $\delta, \delta'$ in either \textbf{while}
%   loop ensures that all \Select[j]{v} will always be in $[0,1]$;
%   furthermore, never mind which way the coin flip comes up, at least
%   one previously fractional \Select[j]{v} will become 0 or 1.
% \item As a result, after the first \textbf{while} loop terminates, for
%   each $v$, at most one \Select[j]{v} is fractional.
  
%   Similarly, after the second \textbf{while} loop terminates,
%   overall, at most one \Select[j]{v} is fractional.
% \item As a result, for each $v$, the first \textbf{while} loop can at
%   most result in increasing $\sum_j \Select[j]{v}$ to the nearest
%   integer.

%   Similarly, the step of rounding the \Select[j]{v} to \ISelect[j]{v}
%   can at most increase $\sum_v \sum_j \Select[j]{v}$ by rounding it to
%   the nearest integer.
% \end{enumerate}

% The preceding discussion implies that the rounded variables
% \ISelect[j]{v} satisfy the third and fourth constraints of
% LP~\eqref{eqn:ILP}.
% The definitions of \ISSel{i} and \IRev[j] ensure that the remaining
% constraints are satisfied, except for the sixth constraint,
% which upper-bounds the revenue from advertiser $j$ by \BUDGET[j].

% It remains to analyze the approximation guarantee for the total revenue.
% Here, the key insight is that each \Select[j]{v} is a Martingale as a
% function of \textbf{while} loop iterations, i.e., the expectation of
% its new value after a rounding step is its current value.
% This is a straightforward two-line expectation calculation;
% see \cite{gandhi:khuller:parthasarathy:srinivasan:dependent}.
% In particular, this implies that
% $\Expect{\ISelect[j]{v}} = \Prob{\ISelect[j]{v} = 1} = \Select[j]{v}$.

% Now consider any set $R_i \in \RRP[j]$.
% With explanations of some steps given below,
% the probability that $\ISSel{i} = 1$ is
% \begin{align*}
%   \Prob{\ISSel{i} = 1}
%   & = 1 - \Prob{\ISelect[j(i)]{v} = 0 \text{ for all } v \in R_i}
% \\  & \stackrel{(1)}{\geq} 1 - \prod_{v \in R_i} \Prob{\ISelect[j(i)]{v} = 0}
% \\  & = 1 - \prod_{v \in R_i} (1-\Select[j(i)]{v})
% \\  & \stackrel{(2)}{\geq} 1 - \e^{-\sum_{v \in R_i} \Select[j(i)]{v}}
% \\  & \geq 1 - \e^{-\min(1, \sum_{v \in R_i} \Select[j(i)]{v})}
% \\  & \stackrel{(3)}{\geq} (1-1/\e) \cdot \min(1, \sum_{v \in R_i} \Select[j(i)]{v})
% \\  & \stackrel{(4)}{\geq} (1-1/\e) \cdot \SSel{i}.
% \end{align*}

% The inequality labeled (1) essentially captures negative correlation.
% The proof is very similar to the analysis of Gandhi et
% al.~\cite{gandhi:khuller:parthasarathy:srinivasan:dependent},
% but because our rounding instance does not precisely fit into their
% framework\footnote{The reason is the 
%   truncation constraint on the combined seed set size,
%   which is in addition to the individual node constraints.},
% we give a self-contained proof in Section~\ref{sec:negative-correlation}.

% The inequality labeled (2) used the standard bound that $1-x \leq
% \e^{-x}$ for all $x \geq 0$.

% The inequality labeled (3) uses that the function
% $x \mapsto 1-\e^{-x}$ is concave,
% and hence on the interval $[0,1]$ is lower-bounded by the straight
% line which agrees with it at the endpoints $x=0$ and $x=1$,
% which is the function $x \mapsto (1-1/\e) \cdot x$.

% Finally, the inequality labeled (4) uses that
% $\SSel{i} \leq \min(1, \sum_{v \in R_i} \Select[j(i)]{v})$
% by the first and second LP constraints.
% Using the definition of \IRev[j], we now get that

% \begin{align*}
%   \Expect{\IRev[j]}
%   & = \Expect{\sum_{i \in \RRP[j]} \PER[j] \cdot \ISSel{i}}
% \\ & = \sum_{i \in \RRP[j]} \PER[j] \cdot \Prob{\ISSel{i} = 1}
% \\ & \geq \sum_{i \in \RRP[j]} \PER[j] \cdot (1-1/\e) \cdot \SSel{i}
% \\ & \geq (1-1/\e) \cdot \Rev[j]       
% \end{align*}



==> conclusions-new.tex <==
We explored the problem of maximizing the host's payoff for a budgeted
multi-advertiser setting with constraints on the ad exposure of
each node and each advertiser's seed set size.  
We showed that under a very general class of influence models,
this problem can be cast as maximizing a submodular function subject
to two matroid constraints.
It can therefore be approximated to within essentially a factor \half
using an algorithm due to
Lee et al.~\cite{lee:sviridenko:vondrak:multiple-matroids};
this improves on the \third-approximation guarantee of
\cite{datta:majumder:shrivastava}.
When there are no constraints on individual advertisers' seed set
sizes, only on the total number of seeds,
the constraints form just a single truncated partition matroid.
Therefore, the algorithm of Vondr\'{a}k et
al.~\cite{calinescu:chekuri:pal:vondrak,vondrak:submodular-welfare}
gives $(1-\frac{1}{\e})$-approximation algorithm, 
while a simple greedy
algorithm~\cite{fischer:nemhauser:wolsey}
achieves a \half-approximation. 
For the special case of the Independent Cascade model,
the Reverse Reachability Technique~\cite{borgs:brautbar:chayes:lucier,%
tang:shi:xiao:martingale,tang:xiao:shi:near-optimal}
can be combined with a linear program and rounding due to
\cite{calinescu:chekuri:pal:vondrak:ipco,gandhi:khuller:parthasarathy:srinivasan:dependent}
to yield a more efficient $(1-1/\e)$-approximation algorithm,
even under both types of constraints.

Our experiments show that in practice, the greedy algorithm slightly
outperforms the LP-rounding based algorithm, despite the worse approximation
guarantee.
They also reveal that competition between advertisers leads to a loss
in payoff for the host when the advertisers' influence networks are
more similar, and particularly so when the networks have few highly
influential nodes --- in that case, these nodes cannot simultaneously
be used as seeds for all advertisers, and 
the average exposure per advertiser becomes significantly lower than
the individual exposures of the advertisers on isolated networks.

Our work was in part motivated by considering a more ``natural''
objective function than the notion of regret from \cite{aslay2015viral}.
If one believes that giving advertisers free exposure is detrimental
to the host company, 
excess exposure could alternatively be modeled as a negative term in
the objective function.
In additional work --- not included here --- we have shown that if
the penalty per unit excess exposure is constant, both the
LP-based approach from Section~\ref{sec:IC} and the greedy algorithm 
will still yield a constant-factor approximation guarantee.

%In additional work --- not included here --- we have shown that if the
%penalty for excess exposure is sufficiently mild, then the LP-based
%approach from Section~\ref{sec:IC} can be modified to still yield a
%constant-factor approximation guarantee.

There are several natural directions for future work.
Perhaps most directly, the LP-rounding based algorithm only satisfies
the budget constraint in expectation;
indeed, we have shown a large integrality gap for the LP.
It is a natural question whether a $(1-1/\e)$-approximation guarantee
can be obtained while always satisfying the budget constraints,
and without invoking the heavy Continuous Greedy machinery discussed
in Section~\ref{sec:general}.

An interesting empirical study would be to evaluate to what extent
influential nodes in one advertiser's network are also influential in other
advertisers' networks.
Within typical social networks, one would expect significant
differences based on individuals' expertise;
on the other hand, the use of celebrities to endorse products entirely
outside their realm of expertise shows that humans appear willing to
project expertise in one area on other areas as well.


==> penalty.tex <==
While our objective for the main part of this submission is to
maximize the network's revenue without any penalties for free exposure, 
in this section, we show that even penalties for overshooting an 
advertiser's budget can be incorporated
into the objective function at a slight loss in approximation
guarantees. We use the terms influence and exposure interchangeably in the following text.

Recall that Aslay et al.~\cite{aslay2015viral} focus on a notion of
\emph{regret}: their goal is to minimize the deviation between the
total value an advertiser receives and the advertiser's budget.
This penalizes deviations above or below the budget.
Here, we instead consider the network's \emph{revenue}, but augment it
by a (negative) penalty term which subtracts the free exposure the
network is offering the advertiser, weighted by a parameter $\beta$.
Notice that this is a ``softer'' form of penalty --- in particular, it
does not rule out approximation guarantees for an algorithm simply
based on its inability to hit the budget exactly.
The revised payoff or objective function is the following:

%\begin{equation}
\begin{multline}
\PEObj{\Active[1]{0}, \Active[2]{0}, \ldots, \Active[m]{0}}
\; = \;
\sum_{j=1}^m \ValFun[j]{\Expect{\FinalSize[j]{\Active[j]{0}}}} - \\
\beta \cdot \sum_{j=1}^m  \max \left(
  \PER[j] \cdot \Expect{\FinalSize[j]{\Active[j]{0}}} - \BUDGET[j], 0 \right).
\label{eqn:penalty}
\end{multline}

The first term on the right-hand side of \eqref{eqn:penalty} is
exactly the revenue as defined in Equation~\eqref{eqn:expect-inside}.
The second term is the free exposure,
scaled by a factor of $\beta \in [0,1]$.
The scaling factor can be used to capture the different importance a
network may ascribe to free exposure;
the case $\beta=0$ is the one treated in the body of the submission,
while $\beta = 1$ corresponds to the penalty assumed by
Aslay et al.~\cite{aslay2015viral}.
Similar to our main problem statement defined in section 
\ref{sec:problem-statement} of the paper, 
we consider the following constraints in this problem as well:
\begin{enumerate}
    \item Seed set size constraint - $\sum_j |\Active[j]{0}| \leq \SBUDGET$.
    \item Node exposure constraint - $\SetCard{\SET{\Active[j]{0} \ni v}} \leq \ExposureBound{v}$.
\end{enumerate}


Our main theorem in this section is the following:
\begin{theorem}
\label{thm:penalty-greedy}
Assume that no single node has an influence more than any advertiser's
budget, that is, $\PER[j] \cdot \FinalSize[j]{\SET{v}} \leq \BUDGET[j]$,
for all nodes $v$ and advertisers $j$.
The greedy algorithm, which always adds the next element maximizing the
increase in the objective function, and stops when no element
has positive marginal payoff,
%until there is at least one element with positive marginal payoff,
%(subject to not violating the seed set constraints),
is a $\frac{1+\beta}{2+3\beta}$ approximation algorithm for maximizing 
$\PEObj{\Active[1]{0}, \Active[2]{0}, \ldots, \Active[m]{0}}$,
subject to the seed set constraint $\sum_j |\Active[j]{0}| \leq \SBUDGET$
and the node exposure constraints
$\SetCard{\SET{\Active[j]{0} \ni v}} \leq \ExposureBound{v}$.
\end{theorem}

Note that due to the negative term (which occurs when
$\PER[j] \cdot\FinalSize[j]{\Active[j]{0}} > \BUDGET[j]$),
the objective function $\PEObj{\cdot}$ is in general neither monotone
nor submodular.
Hence, standard results such as theorem \ref{thm:submodular-multiple-matroids} and
\ref{thm:submodular-greedy} from the main paper do not apply here.

\subsection{Proof Outline}
Before we dive into the details of the proof, we give some intuition into the
derivation. We divide the advertisers into 2 sets and individually prove
the bounds on the payoff of both sets:
\begin{enumerate}[leftmargin=*]
    \item Advertisers getting free exposure $\Camp[]^{OV} \rightarrow$ It is the set of advertisers
    for which the greedily selected seed nodes overshoot their respective
    budgets. For advertisers in $\Camp[]^{OV}$, we leverage the fact that no single node
    individually exerts greater influence than the budgets and that we are
    \textit{greedily} selecting the seeds only until the marginal payoff is positive. 
    
    Using these properties, we compute an upper bound on the amount by which
    the influence may have exceeded the Budget. Since budget is also the upper 
    bound on the optimal payoff of any advertiser, we obtain a lower bound on the
    greedy payoff in terms of the optimal payoff.
    
    \item Advertisers not getting free exposure $\Camp[]^{UN} \rightarrow$ It is the set of 
    advertisers for which the greedily selected seed nodes undershoot their
    respective budgets. For these advertisers, we adopt a different strategy.
    We begin with a solution that is optimal for $\Camp[]^{UN}$. Obviously,
    the payoff of $\Camp[]^{UN}$ will be better under this solution compared to 
    their total payoff under the overall optimal solution. Hence, any bounds
    on greedy's performance wrt this solution can be directly extended to the overall
    optimal solution.
    
    With every greedy selection, we evaluate how much the final payoff can suffer,
    relative to the optimal solution for $\Camp[]^{UN}$ just before the selection.
    By adding up these losses across all the rounds of greedy seed selection, we 
    obtain a bound on the payoff of $\Camp[]^{UN}$.
    
    Note that payoff from an advertiser can suffer due to multiple reasons, 
    such as losing a seed node to another advertiser. When
    free exposure is penalized, the net payoff from an advertiser may decrease even
    by adding a seed to itself if the node was not present in the optimal
    solution. In such a situation, to achieve better upper bound on 
    the loss incurred, we use a trick to drop some of the seeds from
    the current optimal. By using submodularity of influence, we are able
    to estimate the maximum amount of loss that can be resulted by such a seed selection.
\end{enumerate}
Finally, by summing up the individual bounds for $\Camp[]^{OV}$ and $\Camp[]^{UN}$, we 
obtain the approximation factor given in theorem \ref{thm:penalty-greedy}.

\subsection{Proof for Theorem \ref{thm:penalty-greedy}}

Wlog, we will assume that $\PER[j]=1\ \forall\ j\in\{1,2...m\}$. 
Since we are always dealing with the expected influence only, 
for ease of notation, we will use $\FinalSize[j]{\Active[j]{}}$ 
instead of $\Expect{\FinalSize[j]{\Active[j]{}}}$ to denote the 
expected influence of seed set $\Active[j]{}$ for advertiser $j$. 

We first define some frequently used notations in the proof. 
A solution seed set for the multi-advertiser problem is denoted by $\Active[]{}$ 
(without superscript) and it comprises of $\{node, advertiser\}$ 
pairs denoted by $\{v, \Camp[j]\}$ where $v\in V$ and $\Camp[j]$ represents 
advertiser $j$. The seed set of an individual advertiser $\Camp[j]$ is 
denoted by $\Active[j]{}$ and it comprises of the nodes $v$ where the 
ad of $\Camp[j]$ will be published as a sponsored post.

Let the number of rounds/steps taken by the Greedy algorithm to finish 
seed set selection be $T\leq \SBUDGET$ (the algorithm picks one $\{v, \Camp[j]\}$ 
in each round). Note that $T$ can be less than $l$ because once 
the algorithm exceeds the budget for all advertisers, it will terminate 
even if $l$ pairs of nodes and advertisers haven't been selected. 
Let $\Active[]{G}[t_1:t_2]$ be the seeds\footnote{Note that the 
algorithm picks seed node and advertiser both, in each step. For the 
ease of explanation, we refer the $\{node, advertiser\}$ pair 
as a \textit{seed} selected by the algorithm.} picked by the greedy 
algorithm from round $t_1$ to $t_2$\footnote{The rounds are 
1-indexed i.e. the round IDs start from $1$ and end at $T$.} 
and $\Active[j]{G}[t_1:t_2]$ be the seeds selected for $\Camp[j]$ in 
the same interval. We also define a new \textit{payoff} function for the advertisers as follows:

\begin{equation*}
    \PValFun[j]{\Active[j]{0}} = \ValFun[j]{\Active[j]{0}} - \beta\cdot 
    \max{\left(\FinalSize[j]{\Active[j]{0}} - \BUDGET[j], 0 \right)}
\end{equation*}

We divide the advertisers into two sets:
\begin{enumerate}
    \item $\Camp[]^{OV} \rightarrow$ is the set of all advertisers 
    for whom the greedy solution overshoots their respective budgets 
    in expectation i.e. $\Camp[]^{OV} = \cup_J \{\Camp[j]\ |\  \FinalSize[j]{\Active[j]{G}[1:T]} > \BUDGET[j]\}$.
    \item $\Camp[]^{UN} \rightarrow$ is the set of all advertisers 
    for whom the greedy solution undershoots their respective budgets 
    in expectation i.e. $\Camp[]^{UN} = \cup_J \{\Camp[j]\ |\  \FinalSize[j]{\Active[j]{G}[1:T]} \leq \BUDGET[j]\}$.
\end{enumerate}

Clearly, the host incurs penalty for free exposure for advertisers 
in $\Camp[]^{OV}$. We further define \PEObjOv{\Active[]{}} 
and \PEObjUn{\Active[]{}} as the total payoffs of advertisers 
in $\Camp[]^{OV}$ and $\Camp[]^{UN}$, respectively, for the seed 
set $\Active[]{}$. Note that the sets $\Camp[]^{OV}$ and $\Camp[]^{UN}$ 
only depend on the output of the greedy algorithm and are independent 
of the set $\Active[]{}$ in the definition above.

\PValFun[j]{\Active[j]{0}} accounts for the penalty of overshooting 
and represents the overall contribution of $\Camp[j]$ to the new objective function. 
We define a modified version of submodularity called \textit{positive submodularity} as follows:

\begin{definition}
If $\Omega$ is a finite set, then a set function $f : 2^{\Omega}\rightarrow \mathcal{R}$ 
defined on power set of $\Omega$ is positive submodular if for 
every $X\subseteq Y\subseteq \Omega$ and $v\in \Omega \setminus Y$ 
such that $f(X\cup \{v\})-f(X)\geq 0$, it holds that
\begin{equation*}
    f(X\cup \{v\})-f(X) \geq f(Y\cup \{v\})-f(Y)
\end{equation*}
In other words, if the marginal value of an element when added to a 
set $X$ is non-negative, it will only decrease as $X$ increases further.
\end{definition}

Note that $\PVALFUN[j]$ is \textit{positive submodular} for all $j$ because
\begin{itemize}
    \item If adding $v$ to the existing seed set $\Active[j]{0}$ of $j$ 
    does not result in $\FINALSIZE[j]$ overshooting $\BUDGET[j]$, marginal 
    payoff of $v$ is going to decrease with increase in $\Active[j]{0}$ due 
    to submodularity of $\FINALSIZE[j]$.
    
    \item If adding $v$ to the existing seed set $\Active[j]{0}$ of $j$ 
    results in $\FINALSIZE[j]$ overshooting $\BUDGET[j]$ by $r$, marginal 
    payoff of $v$ is going to decrease with increase in $\Active[j]{0}$ 
    because any augmentation to $\Active[j]{0}$ will decrease the marginal 
    revenue of $v$ more than it decreases the marginal penalty of adding 
    $v$\footnote{If augmenting $\Active[j]{0}$ with $\{U\}$ does not 
    result in overshooting, the marginal penalty of adding $v$ to 
    $\Active[j]{0}\cup \{U\}$ will remain the same as adding $v$ to $\Active[j]{0}$, 
    only marginal payoff will decrease. If augmenting $\Active[j]{0}$ 
    with $\{U\}$ does result in overshooting, the marginal payoff of 
    adding $v$ to $\Active[j]{0}\cup \{U\}$ will become non-positive 
    which is not greater than the marginal payoff of adding $v$ to $\Active[j]{0}$}.
\end{itemize}

Let $Q[t]$ be the problem of selecting seeds that maximize $\PEOBJ$ 
given that $t$ seeds have already been selected by the greedy algorithm. 
Let the optimum solution to $Q[t]$ be $\Active[]{*}[t]$. Clearly, 
$\Active[]{*}[0]$ is the optimum solution to the problem of maximizing
 $\PEOBJ{}$. To prove theorem \ref{thm:penalty-greedy}, we have to show that 
\[
    \PEObj{\Active[]{G}[1:T]} = \PEObjUn{\Active[]{G}[1:T]} +  
    \PEObjOv{\Active[]{G}[1:T]} \geq \frac{\beta+1}{3\beta+2}\PEObj{\Active[]{*}[0]}
\]

\begin{lemma}
$\frac{2\beta+1}{\beta+1}\PEObjOv{\Active[]{G}[1:T]} \geq \PEObjOv{\Active[]{*}[0]}$
\label{lemma:ov}
\end{lemma}
\begin{proof}
Consider an advertiser $\Camp[i]\in \Camp[]^{OV}$ and let $X=\Active[i]{G}[1:T]$.
 Let $v$ be the last seed node assigned to $\Camp[i]$ by the greedy algorithm. 
 Since greedy selected $\{v, \Camp[i]\}$ pair, its marginal payoff must have
 been positive. Thus, we can say that $\FinalSize[i]{X\setminus \{v\}} < \BUDGET[i]$ 
 i.e. campaign of $\Camp[i]$ would not have exceeded the budget if $v$ 
 was not chosen. The marginal payoff of $v$ is thus given by:
\begin{align}
    &\left(\BUDGET[i]-\beta\cdot\left(\FinalSize[i]{X}-\BUDGET[i]\right)\right) - 
    \left(\FinalSize[i]{X\setminus\{v\}}\right)  \geq 0 \nonumber \\ 
    &\implies
    \BUDGET[i]\cdot(1+\beta) \geq \beta\FinalSize[i]{X} + \FinalSize[i]{X\setminus\{v\}}
\label{eq:ov1}
\end{align}

Since no vertex has more influence than the budget of advertiser,  
$\FinalSize[i]{X} > \BUDGET[i]$ implies that
$\FinalSize[i]{X\setminus\{v\}}\neq \phi$. Moreover, since $v$ was 
selected after all nodes in $X\setminus\{v\}$, its payoff must have 
been smaller than the payoff of $X\setminus\{v\}$ for $\Camp[i]$. 
From submodularity of $\FinalSize[i]{}$ and equation \ref{eq:ov1}, we can say that
\begin{align}
    &\FinalSize[i]{X} - \FinalSize[i]{X\setminus\{v\}} \leq \FinalSize[i]{v} = 
    \PValFun[i]{v} \leq \PValFun[i]{X\setminus\{v\}} = \FinalSize[i]{X\setminus\{v\}} \nonumber \\
    &\implies \FinalSize[i]{X\setminus\{v\}} \geq \frac{1}{2}\FinalSize[i]{X}
\label{eq:ov2}
\end{align}

From equations \ref{eq:ov1} and \ref{eq:ov2}, we get
\begin{align*}
    \BUDGET[i]\cdot(1+\beta)\geq \FinalSize[i]{X}\cdot\left(\beta + \frac{1}{2}\right) 
    \implies \FinalSize[i]{X} \leq \frac{2(\beta+1)}{2\beta+1}\BUDGET[i]
\end{align*}

Since $\Camp[i]\in \Camp[]^{OV}$, the payoff is given by:
\begin{equation*}
    \PValFun[i]{X} = \BUDGET[i] - \beta\cdot(\FinalSize[i]{X}-\BUDGET[i]) 
    \geq \frac{\beta+1}{2\beta+1}\BUDGET[i] \geq \frac{\beta+1}{2\beta+1}\PValFun[i]{\Active[i]{*}[0]}
%\label{eq:ov3}
\end{equation*}
Adding payoff from all overshooting advertisers $(\Camp[]^{OV})$, we get:
\begin{equation*}
    \PEObjOv{\Active[]{G}[1:T]} \geq \frac{\beta+1}{2\beta+1}\PEObjOv{\Active[]{*}[0]}
\end{equation*}

\end{proof}

Next, we derive the relation between optimal payoff and the payoff for 
greedily chosen seed set for the advertisers in $\Camp[]^{UN}$.

\begin{lemma}
$\frac{3\beta+2}{\beta+1}\PEObjUn{\Active[]{G}[1:T]} + \PEObjOv{\Active[]{G}[1:T]} \geq \PEObjUn{\Active[]{*}[0]} $
\label{lemma:un}
\end{lemma}
\begin{proof}
Consider the $t^{th}$ round of Greedy and let the problem of picking seed sets given $t-1$ rounds of greedy be denoted as $Q[t-1]$. Let us say that the Greedy algorithm picks a 
vertex $v$ and assigns it to $\Camp[i]$, earning a payoff 
$\psi=\PValFun[i]{\Active[i]{G}[1:t}-\PValFun[i]{\Active[i]{G}[1:t-1]}$. 

%Let us say that just before $\{v, \Camp[i]\}$ was selected, $Q[t-1]$ 
%was the problem to 
%solve with optimal solution $\Active[]{*}[t-1]$. 

Let $\ActiveUN[]{*}[t-1]$ be the optimal solution for \textit {advertisers in the set $\Camp[]^{UN}$} after $t-1$ rounds of greedy. Clearly, $\PEObjUn{\ActiveUN[]{*}[0]} \geq \PEObjUn{\Active[]{*}[0]}$. 

%Let the adjusted budgets in $Q[t-1]$  (budget remaining after influence 
%from seeds ti round $t-1$) 

We will evaluate how much a greedy choice in the current 
round can affect 
the optimal payoff for advertisers in $\Camp[]^{UN}$. 

\begin{claim}\label{claim:optOver}
If there exists an advertiser $\Camp[i]\in \Camp[]^{UN}$ such that its seed set under 
optimal solution $\ActiveUN[]{*}[t-1]$ is non-empty and overshoots 
the budget i.e. $\ActiveUN[i]{*}[t-1]\neq \phi$ and 
$\FinalSize[i]{\Active[i]{G}[1:t-1] \cup \ActiveUN[i]{*}[t-1]} > \BUDGET[i]$, 
then removing any node from the seed set of $\Camp[i]$ will either 
have no affect or will prevent the budget overshooting i.e. if $v\in \ActiveUN[i]{*}[t-1]$, then either
\begin{align*}
\FinalSize[i]{\Active[i]{G}[1:t-1] \cup \ActiveUN[i]{*}[t-1]\setminus \{v\}} = 
\FinalSize[i]{\Active[i]{G}[1:t-1] \cup \ActiveUN[i]{*}[t-1]}.
\end{align*}
or
\begin{align*}
\FinalSize[i]{\Active[i]{G}[1:t-1] \cup \ActiveUN[i]{*}[t-1]\setminus \{v\}} \leq \BUDGET[i].
\end{align*}
\end{claim}
\begin{proof}
If removing $v$ has any affect, it can only decrease the exposure. 
However, if the exposure still overshoots the budget after removing $v$, 
then removal of $\{v, \Camp[i]\}$ will improve the overall
payoff of $\Camp[]^{UN}$. This implies that $\ActiveUN[]{*}[t-1]$ is not optimal for $\Camp[]^{UN}$, which is a contradiction.
\end{proof}

Let $\FinalSizeMarg[i]{\Active[i]{}} = \FinalSizeMarg[i]{\Active[i]{G}[1:t-1] \cup \Active[i]{}} 
- \FinalSizeMarg[i]{\Active[i]{G}[1:t-1]}$ be the marginal influence of 
set $\Active[i]{}$ for $\Camp[i]$ after $t-1$ rounds of greedy. Similarly, 
let $\PValFunMarg[i]{\Active[i]{}}$ be the marginal payoff of  $\Active[i]{}$ 
if selected as a seed set for $\Camp[i]$ and $\PEOBJUNMARG$ be the marginal payoff of seed sets for advertisers in $\Camp[]^{UN}$.

When the greedy choice is made, one of the following three cases may occur:
\begin{enumerate}
    \item $\{v, \Camp[i]\} \in \ActiveUN[]{*}[t-1]$ i.e. the optimal solution for $\Camp[]^{UN}$
    also contains the same seed. In this case, there will be no loss of 
    payoff i.e. $\PEObjUnMarg{\ActiveUN[]{*}[t]} + \psi = \PEObjUnMarg{\ActiveUN[]{*}[t-1]}$.
    \item $\ActiveUN[]{*}[t-1]$ also selects $v$ but assigns it to a different (set of) advertiser(s) $\Camp[k]$. Let us build a 
    feasible solution $\Active[]{F}$ for the problem $Q[t]$ by 
    modifying the seed set of only $\Camp[i]$ and $\Camp[k]$ in
    the current optimal $\ActiveUN[]{*}[t-1]$.
    We will analyze the 
    payoff $\PEObjUnMarg{\Active[]{F} \cup \{v, \Camp[i]\}}$.
    Since $\ActiveUN[]{*}[t]$ is optimal for $\Camp[]^{UN}$ after 
    $t$ rounds of 
    greedy, $\PEObjUnMarg{\ActiveUN[]{*}[t] \cup \{v, \Camp[i]\}} 
    \geq \PEObjUnMarg{\Active[]{F} \cup \{v, \Camp[i]\}}$.
    
    We begin with $\Active[]{F} = \ActiveUN[]{*}[t-1]\setminus \{v, \Camp[k]\}$ 
    where $k\neq i$ is such that $\{v, \Camp[k]\} \in \ActiveUN[]{*}[t-1]$. 
    Clearly, this solution satisfies the constraints.
    
    \begin{claim}
    $\PValFunMarg[k]{\Active[k]{F}}$ is at most $\psi$ less than 
    $\PValFunMarg[k]{\ActiveUN[k]{*}[t-1]}$.
    \label{claim:kAd}
    \end{claim}
    \begin{proof}
    The choice of greedy implies that
    $\PValFunMarg[k]{\{v\}}\leq \PValFunMarg[i]{\{v\}}=\psi$. If the 
    optimal solution $\ActiveUN[k]{*}[t-1]$ does not overshoot  budget of $\Camp[k]$, then by submodularity 
    of $\FINALSIZE[k]{}$, we can say that 
    \[
    \FinalSizeMarg[k]{\ActiveUN[k]{*}[t-1]} - \FinalSizeMarg[k]{\ActiveUN[k]{*}[t-1]\setminus\{v\}} = \\
\FinalSizeMarg[k]{v} = \PValFunMarg[k]{v} \leq \psi
    \]
    
    If the optimal solution does overshoot the budget, then by claim 
    \ref{claim:optOver} and positive submodularity of $\PVALFUN[k]{}$, 
    we can say that either
    \[
        \PValFunMarg[k]{\ActiveUN[k]{*}[t-1]} - \PValFunMarg[k]{\ActiveUN[k]{*}[t-1]\setminus\{v\}} = 0 \leq \psi\\
    \]
    or
    \[
        \PValFunMarg[k]{\ActiveUN[k]{*}[t-1]} - \PValFunMarg[k]{\ActiveUN[k]{*}[t-1]\setminus\{v\}} 
        \leq \PValFunMarg[k]{v} \leq \psi\\
    \]
    \end{proof}
    
    \begin{claim}
    If $\Camp[i]\in \Camp[]^{UN}$, there is a 
    feasible solution for which marginal payoff
    of $\Camp[i]$ after $t^{th}$ round of greedy is $\frac{\beta}{1+\beta}\psi + \psi$ 
    less than the current optimal $\PValFunMarg[i]{\ActiveUN[i]{*}[t-1]}$.
    \label{claim:iAd}
    \end{claim}
    \begin{proof}
    The greedy choice of $v$ for $\Camp[i]$ can reduce its payoff if and only if 
    adding $v$ to the seed set of $\Camp[i]$ in the optimal solution leads to 
    overshooting of its budget. In this case, we build a feasible 
    solution $\Active[]{F}$ that satisfies the following condition:
    \begin{equation}
        \BUDGET[i] - \frac{\beta}{1+\beta}\psi \leq \FinalSize[i]{\Active[i]{G}[1:t] 
        \cup \Active[i]{F}} \leq \BUDGET[i] + \frac{1}{1+\beta}\psi
        \label{eq:range}
    \end{equation}
    Since $\Camp[i]\in \Camp[]^{UN}$, the greedy selection of $v$ will not result 
    in exposure for $\Camp[i]$ overshooting $\BUDGET[i]$. Hence, marginal payoff 
    of $\{v, \Camp[i]\}$ is also the marginal influence of $v$ for $\Camp[i]$. 
    By submodularity of influence, we can say that no other node in $\ActiveUN[i]{*}[t-1]$ 
    will have marginal influence greater than $\psi$. 
    
    We start with the seed set $\Active[i]{F}=\ActiveUN[i]{*}[t-1]$ 
    and one-by-one, remove nodes from it until
    $\FINALSIZE[i]$ lies in the range given in equation \ref{eq:range}. Since the width of the range 
    (RHS-LHS) in equation \ref{eq:range} is $\psi$ and 
    removal of each node 
    reduces $\FINALSIZE[i]$ by no more than $\psi$, 
    we are guaranteed to get 
    a solution $\Active[i]{F}$ for which equation \ref{eq:range} is true. Hence, 
    the overall payoff for $\Camp[i]$ is given by:
    \begin{align*}
        & \PValFun[i]{\Active[i]{G}[1:t] \cup \Active[i]{F}}  \geq \BUDGET[i]-\frac{\beta}{1+\beta}\psi \\
        \implies & \PValFunMarg[i]{\Active[i]{F}\cup \{v\}} + \PValFun[i]{\Active[i]{G}[1:t-1]}  
        \geq \BUDGET[i]-\frac{\beta}{1+\beta}\psi\\
        \implies & \PValFunMarg[i]{\Active[i]{F}\cup \{v\}} 
        \geq \PValFunMarg[i]{\ActiveUN[i]{*}[t-1]} - \frac{\beta}{1+\beta}\psi
    \end{align*}

    Combining claim \ref{claim:kAd} and \ref{claim:iAd}, we can say that there exists
    a feasible solution \Active[]{F} such that:
    \begin{align*}
   \PEObjUnMarg{\Active[]{F}\cup \{v,\Camp[i]\}} \geq \left\{
\begin{array}{ll}
     \PEObjUnMarg{\ActiveUN[]{*}[t-1]} - \psi & \text{if}\ \Camp[i]\in \Camp[]^{OV} \\
\PEObjUnMarg{\ActiveUN[]{*}[t-1]} - \psi -\frac{\beta}{1+\beta}\psi & \text{if}\ \Camp[i]\in \Camp[]^{UN} \\
\end{array} 
\right.
\end{align*}
As noted earlier, $\PEObjUnMarg{\ActiveUN[]{*}[t] \cup \{v, \Camp[i]\}} 
    \geq \PEObjUnMarg{\Active[]{F} \cup \{v, \Camp[i]\}}$. Hence, 
    \begin{align}
   \PEObjUnMarg{\ActiveUN[]{*}[t]\cup \{v,\Camp[i]\}} \geq \left\{
\begin{array}{ll}
     \PEObjUnMarg{\ActiveUN[]{*}[t-1]} - \psi & \text{if}\ \Camp[i]\in \Camp[]^{OV} \\
\PEObjUnMarg{\ActiveUN[]{*}[t-1]} - \psi -\frac{\beta}{1+\beta}\psi & \text{if}\ \Camp[i]\in \Camp[]^{UN} \\
\end{array} 
\right.
\label{eq:case2UN}
\end{align}
    

    \end{proof}
    
    \item The optimal solution does not pick $v$.
    The proof and results for this scenario are similar to the previous case.
    
\end{enumerate}

Combining all 3 cases and adding the results for $T$ rounds, we can say that
\begin{align}
   &\PEObjUn{\Active[]{G}[1:T]} \geq \PEObjUn{\ActiveUN[]{*}[0]} - 
   \PEObjOv{\Active[]{G}[1:T]} - \left(1+\frac{\beta}{1+\beta}\right)\PEObjUn{\Active[]{G}[1:T]}
    \nonumber \\ 
    &\implies \frac{3\beta+2}{\beta+1} \PEObjUn{\Active[]{G}[1:T]} +  
    \PEObjOv{\Active[]{G}[1:T]} \geq \PEObjUn{\Active[]{*}[0]}
    \label{eq:un}
\end{align}

because $\ActiveUN[]{*}[0]$ is optimal for advertisers $\Camp[]^{UN}$ and hence, $\PEObjUn{\ActiveUN[]{*}[0]}\geq \PEObjUn{\Active[]{*}[0]}$.

\end{proof}


From lemma \ref{lemma:ov} and \ref{lemma:un}, we get
\begin{align}
    \frac{3\beta+2}{\beta+1}\cdot (\PEObjUn{\Active[]{G}[1:T]} +  \PEObjOv{\Active[]{G}[1:T]}) \geq & \PEObjUn{\Active[]{*}[0]} + \PEObjOv{\Active[]{*}[0]}\nonumber \\ 
    \PEObj{\Active[]{G}[1:T]} \geq &\frac{\beta+1}{3\beta+2}\PEObj{\Active[]{*}[0]}
\end{align}

Hence, the greedy algorithm which always adds the next element maximizing the increase in $\PEOBJ$ and stops when no element has a positive marginal payoff is a $\frac{\beta+1}{3\beta+2}$ approximation algorithm for maximizing $\PEObj{\Active[1]{0}, \Active[2]{0}, \ldots, \Active[m]{0}}$.

